Essential spectrum of the discrete Laplacian on a perturbed periodic graph

We address the Laplacian on a perturbed periodic graph which might not be a periodic graph. We present a class of perturbed graphs for which the essential spectra of the Laplacians are stable even when the graphs are perturbed by adding and removing infinitely many vertices and edges. Using this result, we demonstrate how to determine the spectra of cone-like graphs, the upper-half plane, and graphs obtained from $\mathbb{Z}^2$ by randomly adding vertices.

==> FigEx44.tex <==
%WinTpicVersion4.32a
{\unitlength 0.1in%
\begin{picture}(38.0500,19.1000)(5.9500,-22.9500)%
% LINE 2 0 3 0 Black White  
% 2 1000 1000 4400 1000
% 
\special{pn 8}%
\special{pa 1000 1000}%
\special{pa 4400 1000}%
\special{fp}%
% CIRCLE 2 0 0 0 Black Black  
% 4 1200 1000 1250 1000 1250 1000 1250 1000
% 
\special{sh 1.000}%
\special{ia 1200 1000 50 50 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 1200 1000 50 50 0.0000000 6.2831853}%
% CIRCLE 2 0 0 0 Black Black  
% 4 1800 1000 1850 1000 1850 1000 1850 1000
% 
\special{sh 1.000}%
\special{ia 1800 1000 50 50 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 1800 1000 50 50 0.0000000 6.2831853}%
% CIRCLE 2 0 0 0 Black Black  
% 4 2400 1000 2450 1000 2450 1000 2450 1000
% 
\special{sh 1.000}%
\special{ia 2400 1000 50 50 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 2400 1000 50 50 0.0000000 6.2831853}%
% CIRCLE 2 0 0 0 Black Black  
% 4 3000 1000 3050 1000 3050 1000 3050 1000
% 
\special{sh 1.000}%
\special{ia 3000 1000 50 50 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 3000 1000 50 50 0.0000000 6.2831853}%
% CIRCLE 2 0 0 0 Black Black  
% 4 3600 1000 3650 1000 3650 1000 3650 1000
% 
\special{sh 1.000}%
\special{ia 3600 1000 50 50 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 3600 1000 50 50 0.0000000 6.2831853}%
% CIRCLE 2 0 0 0 Black Black  
% 4 4200 1000 4250 1000 4250 1000 4250 1000
% 
\special{sh 1.000}%
\special{ia 4200 1000 50 50 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 4200 1000 50 50 0.0000000 6.2831853}%
% LINE 2 0 3 0 Black White  
% 2 1200 1000 1080 600
% 
\special{pn 8}%
\special{pa 1200 1000}%
\special{pa 1080 600}%
\special{fp}%
% CIRCLE 2 0 0 0 Black Black  
% 4 1080 600 1130 600 1130 600 1130 600
% 
\special{sh 1.000}%
\special{ia 1080 600 50 50 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 1080 600 50 50 0.0000000 6.2831853}%
% LINE 2 0 3 0 Black White  
% 2 1800 1000 1700 600
% 
\special{pn 8}%
\special{pa 1800 1000}%
\special{pa 1700 600}%
\special{fp}%
% CIRCLE 2 0 0 0 Black Black  
% 4 1700 600 1750 600 1750 600 1750 600
% 
\special{sh 1.000}%
\special{ia 1700 600 50 50 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 1700 600 50 50 0.0000000 6.2831853}%
% LINE 2 0 3 0 Black White  
% 2 2400 1000 2300 600
% 
\special{pn 8}%
\special{pa 2400 1000}%
\special{pa 2300 600}%
\special{fp}%
% CIRCLE 2 0 0 0 Black Black  
% 4 2300 600 2350 600 2350 600 2350 600
% 
\special{sh 1.000}%
\special{ia 2300 600 50 50 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 2300 600 50 50 0.0000000 6.2831853}%
% LINE 2 0 3 0 Black White  
% 2 3000 1000 2900 600
% 
\special{pn 8}%
\special{pa 3000 1000}%
\special{pa 2900 600}%
\special{fp}%
% CIRCLE 2 0 0 0 Black Black  
% 4 2900 600 2950 600 2950 600 2950 600
% 
\special{sh 1.000}%
\special{ia 2900 600 50 50 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 2900 600 50 50 0.0000000 6.2831853}%
% LINE 2 0 3 0 Black White  
% 2 3600 1000 3500 600
% 
\special{pn 8}%
\special{pa 3600 1000}%
\special{pa 3500 600}%
\special{fp}%
% CIRCLE 2 0 0 0 Black Black  
% 4 3500 600 3550 600 3550 600 3550 600
% 
\special{sh 1.000}%
\special{ia 3500 600 50 50 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 3500 600 50 50 0.0000000 6.2831853}%
% LINE 2 0 3 0 Black White  
% 2 4200 1000 4100 600
% 
\special{pn 8}%
\special{pa 4200 1000}%
\special{pa 4100 600}%
\special{fp}%
% CIRCLE 2 0 0 0 Black Black  
% 4 4100 600 4150 600 4150 600 4150 600
% 
\special{sh 1.000}%
\special{ia 4100 600 50 50 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 4100 600 50 50 0.0000000 6.2831853}%
% STR 2 0 3 0 Black White  
% 4 2400 1060 2400 1160 5 0 0 0
% $(0,0)$
\put(24.0000,-11.6000){\makebox(0,0){$(0,0)$}}%
% STR 2 0 3 0 Black White  
% 4 3000 1060 3000 1160 5 0 0 0
% $(1,0)$
\put(30.0000,-11.6000){\makebox(0,0){$(1,0)$}}%
% STR 2 0 3 0 Black White  
% 4 2300 350 2300 450 5 0 0 0
% $(0,1)$
\put(23.0000,-4.5000){\makebox(0,0){$(0,1)$}}%
% STR 2 0 3 0 Black White  
% 4 700 710 700 810 5 0 0 0
% $G$
\put(7.0000,-8.1000){\makebox(0,0){$G$}}%
% STR 2 0 3 0 Black White  
% 4 1800 1060 1800 1160 5 0 0 0
% $(-1,0)$
\put(18.0000,-11.6000){\makebox(0,0){$(-1,0)$}}%
% STR 2 0 3 0 Black White  
% 4 3600 1060 3600 1160 5 0 0 0
% $(2,0)$
\put(36.0000,-11.6000){\makebox(0,0){$(2,0)$}}%
% LINE 2 0 3 0 Black White  
% 2 1000 2200 4400 2200
% 
\special{pn 8}%
\special{pa 1000 2200}%
\special{pa 4400 2200}%
\special{fp}%
% CIRCLE 2 0 0 0 Black Black  
% 4 1200 2200 1250 2200 1250 2200 1250 2200
% 
\special{sh 1.000}%
\special{ia 1200 2200 50 50 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 1200 2200 50 50 0.0000000 6.2831853}%
% CIRCLE 2 0 0 0 Black Black  
% 4 1800 2200 1850 2200 1850 2200 1850 2200
% 
\special{sh 1.000}%
\special{ia 1800 2200 50 50 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 1800 2200 50 50 0.0000000 6.2831853}%
% CIRCLE 2 0 0 0 Black Black  
% 4 2400 2200 2450 2200 2450 2200 2450 2200
% 
\special{sh 1.000}%
\special{ia 2400 2200 50 50 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 2400 2200 50 50 0.0000000 6.2831853}%
% CIRCLE 2 0 0 0 Black Black  
% 4 3000 2200 3050 2200 3050 2200 3050 2200
% 
\special{sh 1.000}%
\special{ia 3000 2200 50 50 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 3000 2200 50 50 0.0000000 6.2831853}%
% CIRCLE 2 0 0 0 Black Black  
% 4 3600 2200 3650 2200 3650 2200 3650 2200
% 
\special{sh 1.000}%
\special{ia 3600 2200 50 50 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 3600 2200 50 50 0.0000000 6.2831853}%
% CIRCLE 2 0 0 0 Black Black  
% 4 4200 2200 4250 2200 4250 2200 4250 2200
% 
\special{sh 1.000}%
\special{ia 4200 2200 50 50 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 4200 2200 50 50 0.0000000 6.2831853}%
% LINE 2 0 3 0 Black White  
% 2 2400 2200 2250 1800
% 
\special{pn 8}%
\special{pa 2400 2200}%
\special{pa 2250 1800}%
\special{fp}%
% CIRCLE 2 0 0 0 Black Black  
% 4 2250 1800 2300 1800 2300 1800 2300 1800
% 
\special{sh 1.000}%
\special{ia 2250 1800 50 50 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 2250 1800 50 50 0.0000000 6.2831853}%
% STR 2 0 3 0 Black White  
% 4 2400 2260 2400 2360 5 0 0 0
% $(0,0)$
\put(24.0000,-23.6000){\makebox(0,0){$(0,0)$}}%
% STR 2 0 3 0 Black White  
% 4 3000 2260 3000 2360 5 0 0 0
% $(1,0)$
\put(30.0000,-23.6000){\makebox(0,0){$(1,0)$}}%
% STR 2 0 3 0 Black White  
% 4 700 1910 700 2010 5 0 0 0
% $G'$
\put(7.0000,-20.1000){\makebox(0,0){$G'$}}%
% STR 2 0 3 0 Black White  
% 4 1800 2260 1800 2360 5 0 0 0
% $(-1,0)$
\put(18.0000,-23.6000){\makebox(0,0){$(-1,0)$}}%
% STR 2 0 3 0 Black White  
% 4 3600 2260 3600 2360 5 0 0 0
% $(2,0)$
\put(36.0000,-23.6000){\makebox(0,0){$(2,0)$}}%
% STR 2 0 3 0 Black White  
% 4 4200 1060 4200 1160 5 0 0 0
% $(3,0)$
\put(42.0000,-11.6000){\makebox(0,0){$(3,0)$}}%
% STR 2 0 3 0 Black White  
% 4 1200 1060 1200 1160 5 0 0 0
% $(-2,0)$
\put(12.0000,-11.6000){\makebox(0,0){$(-2,0)$}}%
% STR 2 0 3 0 Black White  
% 4 1200 2260 1200 2360 5 0 0 0
% $(-2,0)$
\put(12.0000,-23.6000){\makebox(0,0){$(-2,0)$}}%
% LINE 2 0 3 0 Black White  
% 2 2400 2200 2550 1800
% 
\special{pn 8}%
\special{pa 2400 2200}%
\special{pa 2550 1800}%
\special{fp}%
% CIRCLE 2 0 1 0 Black Black  
% 4 2550 1800 2600 1800 2600 1800 2600 1800
% 
\special{sh 0.100}%
\special{ia 2550 1800 50 50 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 2550 1800 50 50 0.0000000 6.2831853}%
% STR 2 0 3 0 Black White  
% 4 2550 1555 2550 1655 5 0 0 0
% $(0,2)$
\put(25.5000,-16.5500){\makebox(0,0){$(0,2)$}}%
% STR 2 0 3 0 Black White  
% 4 4200 2260 4200 2360 5 0 0 0
% $(3,0)$
\put(42.0000,-23.6000){\makebox(0,0){$(3,0)$}}%
% STR 2 0 3 0 Black White  
% 4 2900 350 2900 450 5 0 0 0
% $(1,1)$
\put(29.0000,-4.5000){\makebox(0,0){$(1,1)$}}%
% STR 2 0 3 0 Black White  
% 4 3500 350 3500 450 5 0 0 0
% $(2,1)$
\put(35.0000,-4.5000){\makebox(0,0){$(2,1)$}}%
% STR 2 0 3 0 Black White  
% 4 4100 350 4100 450 5 0 0 0
% $(3,1)$
\put(41.0000,-4.5000){\makebox(0,0){$(3,1)$}}%
% STR 2 0 3 0 Black White  
% 4 1700 350 1700 450 5 0 0 0
% $(-1,1)$
\put(17.0000,-4.5000){\makebox(0,0){$(-1,1)$}}%
% STR 2 0 3 0 Black White  
% 4 1100 350 1100 450 5 0 0 0
% $(-2,1)$
\put(11.0000,-4.5000){\makebox(0,0){$(-2,1)$}}%
% LINE 2 0 3 0 Black White  
% 2 3000 2200 2850 1800
% 
\special{pn 8}%
\special{pa 3000 2200}%
\special{pa 2850 1800}%
\special{fp}%
% CIRCLE 2 0 0 0 Black Black  
% 4 2850 1800 2900 1800 2900 1800 2900 1800
% 
\special{sh 1.000}%
\special{ia 2850 1800 50 50 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 2850 1800 50 50 0.0000000 6.2831853}%
% LINE 2 0 3 0 Black White  
% 2 3000 2200 3150 1800
% 
\special{pn 8}%
\special{pa 3000 2200}%
\special{pa 3150 1800}%
\special{fp}%
% CIRCLE 2 0 1 0 Black Black  
% 4 3150 1800 3200 1800 3200 1800 3200 1800
% 
\special{sh 0.100}%
\special{ia 3150 1800 50 50 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 3150 1800 50 50 0.0000000 6.2831853}%
% LINE 2 0 3 0 Black White  
% 2 3600 2200 3450 1800
% 
\special{pn 8}%
\special{pa 3600 2200}%
\special{pa 3450 1800}%
\special{fp}%
% CIRCLE 2 0 0 0 Black Black  
% 4 3450 1800 3500 1800 3500 1800 3500 1800
% 
\special{sh 1.000}%
\special{ia 3450 1800 50 50 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 3450 1800 50 50 0.0000000 6.2831853}%
% LINE 2 0 3 0 Black White  
% 2 3600 2200 3750 1800
% 
\special{pn 8}%
\special{pa 3600 2200}%
\special{pa 3750 1800}%
\special{fp}%
% CIRCLE 2 0 1 0 Black Black  
% 4 3750 1800 3800 1800 3800 1800 3800 1800
% 
\special{sh 0.100}%
\special{ia 3750 1800 50 50 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 3750 1800 50 50 0.0000000 6.2831853}%
% LINE 2 0 3 0 Black White  
% 2 4200 2200 4050 1800
% 
\special{pn 8}%
\special{pa 4200 2200}%
\special{pa 4050 1800}%
\special{fp}%
% CIRCLE 2 0 0 0 Black Black  
% 4 4050 1800 4100 1800 4100 1800 4100 1800
% 
\special{sh 1.000}%
\special{ia 4050 1800 50 50 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 4050 1800 50 50 0.0000000 6.2831853}%
% LINE 2 0 3 0 Black White  
% 2 4200 2200 4350 1800
% 
\special{pn 8}%
\special{pa 4200 2200}%
\special{pa 4350 1800}%
\special{fp}%
% CIRCLE 2 0 1 0 Black Black  
% 4 4350 1800 4400 1800 4400 1800 4400 1800
% 
\special{sh 0.100}%
\special{ia 4350 1800 50 50 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 4350 1800 50 50 0.0000000 6.2831853}%
% LINE 2 0 3 0 Black White  
% 2 1800 2200 1650 1800
% 
\special{pn 8}%
\special{pa 1800 2200}%
\special{pa 1650 1800}%
\special{fp}%
% CIRCLE 2 0 0 0 Black Black  
% 4 1650 1800 1700 1800 1700 1800 1700 1800
% 
\special{sh 1.000}%
\special{ia 1650 1800 50 50 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 1650 1800 50 50 0.0000000 6.2831853}%
% LINE 2 0 3 0 Black White  
% 2 1200 2200 1050 1800
% 
\special{pn 8}%
\special{pa 1200 2200}%
\special{pa 1050 1800}%
\special{fp}%
% CIRCLE 2 0 0 0 Black Black  
% 4 1050 1800 1100 1800 1100 1800 1100 1800
% 
\special{sh 1.000}%
\special{ia 1050 1800 50 50 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 1050 1800 50 50 0.0000000 6.2831853}%
% STR 2 0 3 0 Black White  
% 4 3150 1555 3150 1655 5 0 0 0
% $(1,2)$
\put(31.5000,-16.5500){\makebox(0,0){$(1,2)$}}%
% STR 2 0 3 0 Black White  
% 4 3750 1555 3750 1655 5 0 0 0
% $(2,2)$
\put(37.5000,-16.5500){\makebox(0,0){$(2,2)$}}%
% STR 2 0 3 0 Black White  
% 4 4350 1555 4350 1655 5 0 0 0
% $(3,2)$
\put(43.5000,-16.5500){\makebox(0,0){$(3,2)$}}%
\end{picture}}%

